FieryGS: In-the-Wild Fire Synthesis with Physics-Integrated Gaussian Splatting

We consider the problem of synthesizing photorealistic, physically plausible combustion effects in in-the-wild 3D scenes. Traditional CFD and graphics pipelines can produce realistic fire effects but rely on handcrafted geometry, expert-tuned parameters, and labor-intensive workflows, limiting their scalability to the real world. Recent scene modeling advances like 3D Gaussian Splatting (3DGS) enable high-fidelity real-world scene reconstruction, yet lack physical grounding for combustion. To bridge this gap, we propose FieryGS, a physically-based framework that integrates physically-accurate and user-controllable combustion simulation and rendering within the 3DGS pipeline, enabling realistic fire synthesis for real scenes. Our approach tightly couples three key modules: (1) multimodal large-language-model-based physical material reasoning, (2) efficient volumetric combustion simulation, and (3) a unified renderer for fire and 3DGS. By unifying reconstruction, physical reasoning, simulation, and rendering, FieryGS removes manual tuning and automatically generates realistic, controllable fire dynamics consistent with scene geometry and materials. Our framework supports complex combustion phenomena -- including flame propagation, smoke dispersion, and surface carbonization -- with precise user control over fire intensity, airflow, ignition location and other combustion parameters. Evaluated on diverse indoor and outdoor scenes, FieryGS outperforms all comparative baselines in visual realism, physical fidelity, and controllability. Project page can be found at https://pku-vcl-geometry.github.io/FieryGS/.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


Synthesizing realistic, dynamic combustion effects in open-world scenes is widely demanded in AR/VR, gaming, and \cmy{film industry. Beyond entertainment, } applications such as virtual fire drills, robotics perception in adverse conditions, and emergency response training require combustion effects that are not only visually convincing but also physically plausible, aligned with real-world scenes, and interactively controllable.
% cmy: align with our contribution. answers why ours is better than traditional simulation and AutoVFX。
%
Nevertheless, accurately modeling combustion remains highly challenging, as it involves turbulent flame-and-smoke dynamics and participating-media radiative transfer, which are nonlinear, tightly coupled, and temporally evolving.
%
These dynamics are deeply influenced by the surrounding environment: flames propagate along combustible materials, generate volumetric smoke and illumination, and leave carbonized residues on surfaces.
%
Simulating and rendering such complex interactions in a physically grounded and visually authentic manner—especially for in-the-wild scenes—remains an open problem.


%Conduct realistic fire synthesis for arbitrary open-world scenes depends on two critical components: precise scene modeling and accurate physics simulation. While modern graphics engines can generate plausiable fire effects, they require extensive manual effort—crafting 3D models, tuning material parameters, and designing simulation workflows—making them impractical for automatic deployment in diverse, real-world environments. 
%
% Recent scene modeling advances, such as Neural Radiance Fields (NeRF)~\citep{mildenhall2020_nerf} and 3D Gaussian Splatting (3DGS)~\citep{kerbl2023_3dgs}, enable high-fidelity 3D reconstruction from multi-view images. Hpwever, xxx

Realistic fire synthesis in arbitrary open-world scenes relies on two key components: precise scene modeling and accurate physics simulation. While modern graphics engines can generate plausible fire effects, they require extensive manual effort—crafting 3D geometry, tuning material parameters, and designing simulation workflows—rendering them impractical for scalable deployment in diverse real-world settings.
% 
Recent advances in scene modeling, such as Neural Radiance Fields (NeRF)~\citep{mildenhall2020_nerf} and 3D Gaussian Splatting (3DGS)~\citep{kerbl2023_3dgs}, enable high-fidelity 3D reconstruction from multi-view images. However, these methods focus primarily on static appearance and geometry, lacking the physical grounding required for simulating combustion phenomena.
%
% Prior efforts have explored combining physical properties with visual cues~\citep{pacnerf, cai2024gic,li2023climatenerf, feng2024splashing, dai2025rainygs,hsu2024autovfx}, but they may focus on distinct physical environemnts, lack physically coherence, or it falls short in providing precise spatiotemporal control. 
Prior efforts have explored combining physical properties with visual cues~\citep{pacnerf, cai2024gic, li2023climatenerf, feng2024splashing, dai2025rainygs, hsu2024autovfx}, but they either target different physical phenomena, lack \cmy{spatio-temporal }physical consistency, or fail to provide precise spatiotemporal control required for realistic \cmy{and interactive }combustion synthesis.
\begin{comment}

Several works estimate physical properties of these reconstructions from visual cues~\citep{pacnerf, cai2024gic} or generative priors~\citep{huang2024dreamphysics}. \cmy{Relying on differentiable physics solvers, such frameworks with considerable computational overhead are impractical for complex combustion scenarios.} 
% but they are not naturally compatible with combustion simulation.
%
Other efforts have explored the integration of physical simulation with learned scene representations. ClimateNeRF~\citep{li2023climatenerf} couples NeRF 
% with static weather simulations
with procedural modeling of weather effects, % cmy: not entirely static, but no simulation envolved
while Gaussian Splashing~\citep{feng2024splashing} and RainyGS~\citep{dai2025rainygs} simulate liquid interactions like water and rain on 3DGS. 
% \tnx{However, these methods are designed for specific simulation contexts and are not applicable to combustion phenomena.}
\cmy{However, combustion is more sensitive to scene composition, posing a greater challenge than effects addressed in prior work.}
%However, these methods focus on passive or low-energy dynamics and cannot handle the thermodynamic complexity of combustion. 
AutoVFX~\citep{hsu2024autovfx} integrates language control, scene modeling, and Blender~\citep{blender} built-in physics engine, supporting flames and smoke.
% , but it is not tailored for combustion simulation and offers limited parameter control.
\cmy{
However, its dynamics are primarily governed by prompts and corresponding scripts generated by language models, rather than by physically grounded spatiotemporal interactions. This “language-driven” strategy may lack physical coherence compared to scene-driven approaches—e.g., a “fireball” prompt renders visually corresponding results but won't ignite nearby combustible objects existing in the scene. Likewise, it falls short in providing precise spatiotemporal control.} 
% (a fireball fails to ignite a wooden desk), render it less usable for fire safety but more convenient as a video effects generation.


Several works estimate physical properties of these reconstructions from visual cues~\citep{pacnerf, cai2024gic} or generative priors~\citep{huang2024dreamphysics}. \cmy{Relying on differentiable physics solvers, such frameworks with considerable computational overhead are impractical for complex combustion scenarios.} 
%
Other efforts have explored the integration of physical simulation with learned scene representations. ClimateNeRF~\citep{li2023climatenerf} couples NeRF 
with procedural modeling of weather effects, 
while Gaussian Splashing~\citep{feng2024splashing} and RainyGS~\citep{dai2025rainygs} simulate liquid interactions like water and rain on 3DGS. 
%
\cmy{However, combustion is more sensitive to scene composition, posing a greater challenge than effects addressed in prior work.}
%
AutoVFX~\citep{hsu2024autovfx} integrates language control, scene modeling, and Blender~\citep{blender} built-in physics engine, supporting flames and smoke.
%
\cmy{
However, its dynamics are primarily governed by prompts and corresponding scripts generated by language models, rather than by physically grounded spatiotemporal interactions. This “language-driven” strategy may lack physical coherence compared to scene-driven approaches—e.g., a “fireball” prompt renders visually corresponding results but won't ignite nearby combustible objects existing in the scene. Likewise, it falls short in providing precise spatiotemporal control.} 

\end{comment}

% To address these gaps, we propose {\name}, a physically-based framework that integrates 3D Gaussian Splatting with combustion simulation to automatically generate photorealistic, dynamic fire in arbitrary reconstructed scenes, while giving users precise control over ignition, wind direction, flame spread, etc. 
% To address these issues, we propose {\name},  a physically-based framework that integrates physically-accurate and user-controllable combustion simulation inside 3DGS pipeline. 
%
% Our method automatically generates photorealistic, dynamic fire in arbitrary reconstructed scenes, while allowing users to precisely control ignition, wind direction, and flame spread.
%
To address these challenges, we propose {\name}, a physically based framework that integrates accurate and controllable combustion simulation into the 3DGS pipeline.
%
Our method automatically generates photorealistic, dynamic fire in reconstructed scenes while allowing precise control over fire intensity, airflow, ignition location and other combustion parameters.
%
The core of {\name} is the combination of three tightly integrated modules: (1) multimodal large-language-model-based material reasoning, (2) efficient volumetric combustion simulation, and (3) a unified renderer for fire and 3DGS.
%
% This tight coupling of material understanding, physics, and rendering eliminates tedious manual tuning and enables realistic, physically grounded fire effects aligned with scene geometry and materials.

%
% At the core of our method is the seamless integration of 3 important modules: (1) the multimodal large-language-model (LLM) -based physical material reasoning, (2) the efficient volumetric combustion simulation, and (3) a unified renderer for joint rendering of fire and 3DGS.
%
% Such tight coupling of physical understanding, simulation, and rendering not only eliminates the need for tedious manual tuning but also yields realistic and controllable fire dynamics aligned with real-world scene geometry and materials.

Specifically, our pipeline begins by building a 3DGS model that reconstructs geometry, appearance, and key material properties for combustion. 
%
% Then, we employ a physics-driven fire simulator and renderer to add flame and smoke propagation, object charring, \cmy{self-emissive lighting, and direct illumination.}
%and self-emissive lighting. 
% %
% To enrich high-frequency details such as fine flame and smoke structure and \cmy{indirect illumination}, % complex reflections, 
% we further apply a diffusion-based video-to-video generative model for refinement.
%
% \cmy{repeating the first sentence}
% By combining accurate scene modeling, robust physics simulation, and rendering, {\name} delivers fire effects that are both physically plausible and visually compelling, with flexible user control.
% 
% Technically, building an automatic 3DGS combustion simulation framework is highly non-trivial. 
%\cmy{Fig.~\ref{fig:teaser} shows the main techniques integrated in {\name}:}
% To reason about material properties, we leverage the emergent physical understanding capabilities of Multimodal Large Language Models (MLLMs). We segment the 3DGS model using 2D segmentations from SAM~\citep{kirillov2023segment} and prompt GPT-4o~\citep{hurst2024gpt4o} to zero-shot infer combustion-relevant properties from 2D views, then lift these labels into 3D.
To reason about material properties, we leverage the emergent physical understanding capabilities of Multimodal Large Language Models (MLLMs), and prompt GPT-4o~\citep{hurst2024gpt4o} to zero-shot infer combustion-relevant properties for the 3DGS scenes. % views, then lift these labels into 3D.
%
For combustion dynamics, we build on a physically grounded fire model~\citep{nguyen2007gpu}, and extend it for wood charring, {delivering efficient and accurate dynamics.} 
% resulting in an efficient and physically grounded solver.
% capable of simulating turbulent flames and carbonization. \cmy{repeated}
%
% To support accurate and efficient rendering, we derive a unified volume rendering formulation that integrates fire and smoke into the Gaussian splatting pipeline, capturing self-emission and reflections.
{We also present a unified volume rendering formulation that combines fire and smoke with 3D Gaussian Splatting in a seamless rendering framework, enabling realistic self-emission and fire-induced direct illumination of the scene.}
%
% Finally, to enhance high-frequency visual details while maintaining simulation consistency, we apply a pre-trained video-to-video diffusion model for generative refinement. Guided by coarse simulation and rendering outputs, this module enriches fine flame filaments, dense smoke wisps, and realistic secondary lighting.
%
{Tightly coupling these modules allows accurate fire effects to emerge directly from real-world data, without requiring expert design or handcrafted inputs.}
% cmy: adding abundant secondary lighting effects other than direct fire-illumination, and natural high fidelity beyond the simulation and rendering resolution. 

To the best of our knowledge, {\name} is the first framework capable of generating visually and physically realistic combustion for in-the-wild scenes, with precise control over ignition location, fire intensity, airflow, and other combustion parameters. Experiments across tabletop, indoor, and outdoor scenes show that {\name} outperforms the state-of-the-art  baselines
% autoVFX~\citep{}, video generation model, and text-driven 3D editing baselines
in visual realism, physical faithfulness, and user controllability.

\begin{figure*}
    \centering
    \includegraphics[width=1.00\linewidth,height=2.5in]{img/teaser/teaser5.pdf}
    \caption{\small
    {\name} synthesizes physically-grounded fire effects from multi-view image,
    % by seamlessly combining LLM-based scene understanding, physics-based dynamic simulation, and volumetric rendering
    enabling controllable and realistic fire in open-world environments.}
    \label{fig:teaser}
    % simple: RainyGS, complex: slice => playground, kitchen
    \vspace{-1.5em}
\end{figure*}



